Consumption and capital growth

Capital growth, at large scales only, arrives with no help from net saving, and consequently with no help from consumption constraint. Net saving, at large scales, is sacrifice of consumption with nothing in return.

==> tables/tbl-3.tex <==
2021 & -0.33 & 0.09 & -0.18 & 0.08 & 0.08 & 0.06 & -0.03 & 0.06 & -0.31 & 0.02 & -0.33 & 0.01 & -0.05 & 0.06\\ 
2020 & 0.23 & 0.11 & -0.52 & -0.03 & -0.53 & 0.04 & -2.04 & 0.04 & -2.05 & -0.01 & -0.40 & -0.02 & -1.58 & -0.00\\ 
2019 & 0.22 & 0.05 & -0.15 & 0.02 & 5.86 & 0.07 & 0.10 & 0.05 & -0.23 & -0.00 & 1.84 & 0.02 & -0.26 & -0.00\\ 
2018 & -0.20 & 0.03 & -0.07 & -0.00 & -1.58 & 0.07 & -0.29 & 0.03 & 0.22 & -0.01 & -0.26 & 0.02 & 0.03 & 0.01\\ 
2017 & 0.07 & 0.07 & 1.76 & 0.04 & 1.97 & 0.08 & 0.05 & 0.04 & -0.36 & -0.00 & -0.07 & 0.01 & -0.12 & 0.02\\ 
2016 & -0.31 & 0.03 & -0.23 & 0.04 & 1.09 & 0.07 & -0.11 & 0.03 & -0.80 & -0.02 & -0.01 & 0.04 & -0.22 & -0.01\\ 
2015 & -0.34 & 0.05 & 0.12 & 0.07 & 0.71 & 0.06 & -1.44 & -0.01 & -1.28 & -0.02 & -0.15 & 0.02 & -0.16 & -0.01\\ 
2014 & -2.08 & 0.08 & 0.11 & 0.04 & 12.81 & 0.05 & 0.12 & -0.01 & 0.39 & -0.03 & -0.25 & -0.01 & -0.32 & 0.02\\ 
2013 & 0.03 & 0.09 & -0.17 & 0.02 & 0.23 & 0.05 & -0.35 & -0.00 & -0.17 & -0.02 & -0.22 & -0.04 & -0.11 & 0.03\\ 
2012 & -0.09 & 0.02 & -1.23 & -0.00 & -0.13 & 0.03 & -0.11 & -0.01 & -0.96 & -0.01 & -0.01 & -0.08 & -1.51 & -0.00\\ 
2011 & -0.44 & 0.00 & -0.14 & 0.00 & -0.66 & 0.01 & -0.63 & 0.02 & 0.31 & -0.00 & -0.00 & -0.02 & 0.86 & -0.01\\ 
2010 & -0.28 & -0.01 & -0.01 & 0.06 & -0.18 & 0.02 & -0.12 & 0.04 & -0.45 & -0.00 & -0.15 & 0.00 & -0.23 & 0.00\\ 
2009 & 0.51 & -0.13 & -1.55 & -0.07 & -0.29 & -0.00 & 0.68 & -0.04 & -0.41 & -0.02 & -0.04 & -0.08 & 0.06 & -0.04\\ 
2008 & -0.00 & -0.10 & -0.00 & -0.08 & -0.32 & 0.03 & -0.10 & -0.03 & -0.12 & -0.01 & -0.07 & 0.00 & -0.04 & -0.02\\ 
2007 & -0.22 & 0.03 & -0.03 & 0.05 & 0.17 & 0.04 & -0.47 & 0.08 & -0.26 & 0.04 & -0.95 & 0.08 & -0.09 & 0.02\\ 
2006 & -0.55 & 0.07 & -0.23 & 0.02 & -0.39 & 0.02 & -1.18 & 0.11 & 1.12 & 0.10 & -0.28 & 0.08 & 0.07 & 0.03\\ 
2005 & -0.97 & 0.08 & 5.15 & 0.06 & -0.16 & 0.01 & 1.99 & 0.12 & 0.11 & 0.09 & -1.09 & 0.12 & -0.14 & 0.02\\ 
2004 & -0.01 & 0.10 & 1.57 & 0.06 & -0.20 & 0.00 & 0.34 & 0.11 & 0.37 & 0.05 & 0.83 & 0.13 & -0.88 & 0.00\\ 
2003 & -0.23 & 0.03 & -0.02 & 0.06 & -1.52 & -0.01 & 0.05 & 0.08 & 0.17 & 0.04 & 0.33 & 0.12 & -0.24 & -0.00\\ 
2002 & 0.35 & -0.02 & -0.13 & 0.02 & 0.06 & -0.02 & 1.66 & 0.03 & -2.00 & 0.02 & 0.74 & 0.09 & 2.49 & -0.02\\ 
2001 & -0.09 & 0.00 & -0.12 & 0.03 & -0.13 & -0.00 & -0.27 & 0.03 & -0.22 & 0.02 & -0.73 & 0.07 & 0.13 & -0.02\\ 
2000 & -0.19 & 0.05 & 1.24 & 0.08 & -0.80 & 0.05 & -0.78 & 0.08 & -0.73 & 0.04 & -0.57 & 0.09 & 0.04 & 0.01\\ 
1999 & -2.03 & 0.12 & -0.36 & 0.08 & 0.01 & 0.06 & 0.01 & 0.10 & -0.51 & 0.04 & 0.15 & 0.10 & 0.01 & 0.01\\ 
1998 & 0.34 & 0.12 & 0.04 & 0.10 & 0.13 & 0.03 & -0.48 & 0.03 & -2.40 & 0.05 & 0.03 & 0.07 & 2.38 & -0.00\\ 
1997 & 0.63 & 0.09 & -0.30 & 0.06 & -0.33 & 0.01 & 0.44 & 0.05 & -0.03 & 0.06 & -0.13 & 0.05 & 0.33 & -0.00\\ 
1996 & 0.10 & 0.07 & -0.21 & 0.01 & 0.18 & 0.04 & -0.10 & 0.04 & -0.19 & 0.02 & -0.10 & 0.01 & -0.05 & 0.01\\ 
1995 & 0.00 & 0.04 & 0.10 & -0.05 & -0.32 & 0.02 & -0.35 & 0.01 & 1.12 & -0.04 &  & 0.02 & -0.17 & 0.03\\ 
1994 & 8.95 & 0.02 & -0.28 & 0.03 & -0.35 & 0.02 & -1.22 & -0.01 & -0.07 & -0.03 &  & 0.01 & -0.14 & 0.02\\ 
1993 & -16.25 & 0.02 & -0.04 & 0.01 & -0.20 & -0.00 & -1.46 & -0.02 & -0.48 & 0.05 &  & -0.01 & -0.37 & -0.03\\ 
1992 & -0.57 & 0.02 & -0.42 & -0.00 & -0.33 & 0.03 & 0.13 & -0.02 & 4.24 & 0.09 &  & -0.04 & 0.10 & -0.05\\ 
1991 & -0.16 & 0.00 & 0.47 & -0.03 & -0.73 & 0.06 & -0.17 & 0.00 & -0.52 & 0.09 &  & 0.06 & -0.06 & -0.01\\ 
1990 & -0.14 & 0.01 & -0.06 & -0.02 & 33.67 & 0.02 & -0.36 & 0.04 & 2.51 & 0.14 &  & 0.05 & -0.18 & 0.08\\ 
1989 & -0.16 & 0.06 & -0.54 & 0.07 & 0.02 & 0.02 & 0.04 & 0.07 & -0.04 & 0.13 &  & 0.12 & -0.25 & 0.11\\ 
1988 & -0.05 & 0.02 & -0.01 & 0.09 & -0.21 & 0.03 & 0.01 & 0.04 & 1.80 & 0.02 &  & 0.14 & -0.40 & 0.16\\ 
1987 & -0.26 & 0.03 & -0.44 & 0.03 & -0.25 & 0.02 & -0.20 & 0.03 & 0.10 & 0.02 &  & 0.12 & 0.09 & 0.20\\ 
1986 & 0.03 & 0.08 & -0.15 & 0.10 & -0.20 & -0.00 & 0.26 & 0.01 & -0.21 & 0.04 &  & 0.04 & 0.09 & 0.10\\ 
1985 & -0.26 & 0.05 & -0.44 & 0.03 & -0.42 & 0.03 & 1.13 & 0.01 & -2.77 & -0.01 &  & 0.05 & -0.13 & 0.05\\ 
1984 & 0.03 & 0.02 & 0.27 & 0.06 & 1.78 & 0.04 & -0.65 & 0.01 & -2.41 & -0.01 &  & -0.02 & -0.21 & 0.03\\ 
1983 & -0.41 & 0.04 & -0.25 & 0.05 & -0.98 & 0.04 & -0.37 & 0.00 & -0.13 & -0.02 &  & -0.03 & -0.16 & 0.05\\ 
1982 & -0.24 & -0.00 & -0.26 & 0.01 & -1.09 & 0.05 & 0.16 & -0.01 & -0.33 & 0.03 &  & -0.03 & -0.22 & 0.06\\ 
1981 & -0.31 & 0.03 & -0.37 & 0.04 & 0.32 & 0.06 & -0.02 & 0.02 & -2.10 & 0.11 &  & 0.00 & -0.38 & 0.08\\ 
1980 & 91.83 & 0.08 & -0.25 & -0.00 & 0.11 & 0.04 & -0.49 & 0.04 &  & 0.12 &  & -0.00 &  & 0.12\\ 
Avg.\footnotemark & 3.11 & 0.05 & 0.48 & 0.04 & 1.66 & 0.03 & 0.50 & 0.04 & 0.88 & 0.04 & 0.37 & 0.05 & 0.37 & 0.04

==> tables/tbl-5.tex <==

\begin{tabular}{llrrrr}
\toprule
Country & Period & $\theta_{c1}$ & $\theta_{c2}$ & $\theta_{c3}$ & $\theta_{c4}$\\
\midrule
Armenia & 1998 - 2020 (17) & 2.09 & -0.18 & -0.10 & 3.57\\
Aruba & 1997 - 2001 (5) & 74982.54 & 0.73 & -7.44 & -8.42\\
Australia & 1980 - 2018 (28) & 109.25 & -0.16 & -0.11 & -14.67\\
Austria & 1998 - 2021 (13) & 14.85 & -0.08 & -0.09 & 1.97\\
Azerbaijan & 1997 - 2020 (21) & 7.82 & -1.48 & -1.40 & -33.31\\
\addlinespace
Bahrain & 2010 - 2013 (4) & 54.83 & -7.54 & -0.32 & -0.90\\
Belgium & 1997 - 2021 (14) & -2.20 & 0.22 & -0.06 & -1.70\\
Bolivia & 2000 - 2014 (11) & -0.85 & 0.27 & -0.12 & -2.40\\
Botswana & 1997 - 1999 (3) & 4.48 & -0.94 & -0.15 & 11.32\\
Brazil & 1998 - 2019 (18) & 4.63 & -1.09 & -0.21 & -330.89\\
\addlinespace
British Virgin Islands & 1997 - 1998 (2) & 70634.35 & 10.36 & 3.20 & 4.24\\
Bulgaria & 1997 - 2016 (11) & 0.47 & -0.15 & -0.20 & 0.78\\
Burkina Faso & 2001 - 2019 (16) & 19.60 & -0.20 & -0.28 & 1.26\\
Cameroon & 1997 - 2019 (19) & -1.35 & -0.84 & -1.71 & 5.57\\
Canada & 1980 - 2022 (32) & 300.59 & -0.16 & -0.11 & 4.80\\
\addlinespace
Cape Verde & 2009 - 2016 (7) & -28.31 & 0.83 & -0.81 & -2.17\\
Chile & 1998 - 2021 (18) & 5.98 & -0.84 & -0.48 & -2.53\\
China & 1993 - 2020 (23) & -1.20 & 0.21 & -0.05 & 2.89\\
Colombia & 1997 - 2022 (18) & 1.96 & 1.59 & -1.39 & -0.20\\
Costa Rica & 2014 - 2020 (5) & 3387.44 & -1.59 & -0.28 & -8.04\\
\addlinespace
Croatia & 1997 - 2021 (21) & -3303.72 & 1.07 & -1.10 & -3.57\\
Curaçao & 2002 - 2016 (12) & -14.45 & -0.05 & 0.71 & -8.10\\
Cyprus & 1997 - 2021 (23) & 0.84 & -0.22 & -0.16 & -1.02\\
Czechia & 1996 - 2018 (14) & -43.29 & 0.05 & 0.01 & -0.28\\
Côte d’Ivoire & 1997 - 2000 (4) & -3.04 & -1.01 & -0.05 & 0.55\\
\addlinespace
Denmark & 1997 - 2022 (22) & 40.37 & 6.53 & -0.14 & -23.89\\
Dominican Republic & 2007 - 2015 (8) & -1.91 & -0.20 & -0.38 & -2.42\\
Ecuador & 2009 - 2020 (12) & -122.41 & -0.83 & -0.91 & 0.11\\
Egypt & 1998 - 2015 (16) & 6.05 & 1.87 & -1.14 & 3.84\\
El Salvador & 2016 - 2019 (4) & 6161.40 & -3.16 & 3.32 & -3.17\\
\addlinespace
Estonia & 1997 - 2021 (17) & 2.42 & 1.54 & -0.10 & 0.33\\
Finland & 1997 - 2021 (18) & 714.26 & -1.00 & -0.20 & 2.91\\
France & 1980 - 2021 (26) & 3.46 & -0.15 & -0.17 & -3.07\\
Germany & 1980 - 2022 (22) & -1.15 & -0.16 & -0.12 & 1.90\\
Greece & 1997 - 2021 (24) & 53.80 & 0.07 & -0.47 & 21.30\\
\addlinespace
Guatemala & 2003 - 2021 (11) & 4.16 & -3.46 & -0.32 & 1.83\\
Guinea & 2005 - 2010 (4) & -3.61 & -2.17 & -0.34 & 0.04\\
Honduras & 2003 - 2015 (9) & -2087.21 & -0.54 & -0.14 & 0.29\\
Hong Kong & 1997 - 2011 (13) & -2.26 & -1.41 & -0.25 & -7.82\\
Hungary & 1997 - 2021 (17) & -17.24 & -0.27 & -0.06 & -12.18\\
\addlinespace
Iceland & 2002 - 2014 (12) & 53.24 & -0.18 & -0.12 & -5.61\\
India & 2001 - 2019 (13) & -0.81 & 0.46 & 0.01 & 2.56\\
Indonesia & 2019 - 2019 (1) & 27.95 & -3.34 & 0.02 & -0.05\\
Iran & 1998 - 2017 (17) & -2.68 & 1.46 & -0.09 & 4.01\\
Ireland & 1997 - 2021 (20) & 1074830.68 & -4.96 & -0.24 & -2.51\\
\addlinespace
Israel & 1997 - 2017 (18) & -14.31 & 0.11 & -0.72 & -3.43\\
Italy & 1981 - 2021 (19) & -3.33 & -0.21 & -0.10 & 0.99\\
Japan & 1981 - 2021 (25) & 3.25 & 0.06 & -0.11 & -2.09\\
Kazakhstan & 1997 - 2022 (22) & -29.52 & 0.33 & -0.13 & 0.23\\
Kuwait & 2005 - 2017 (10) & 1252.78 & -0.96 & -0.12 & -0.60\\
\addlinespace
Kyrgyzstan & 1998 - 2021 (21) & 0.70 & -0.88 & -0.27 & 8.74\\
Latvia & 1998 - 2021 (18) & 350.79 & -0.27 & -0.12 & 16.46\\
Lithuania & 1997 - 2021 (16) & -2.67 & -0.43 & -0.18 & -1.07\\
Luxembourg & 1998 - 2021 (21) & -0.84 & 0.01 & -0.02 & -0.70\\
Malaysia & 2008 - 2015 (7) & -5.37 & -0.94 & -0.19 & -0.57\\
\addlinespace
Malta & 1997 - 2021 (20) & 394.38 & -0.24 & -0.05 & 0.05\\
Mauritius & 2015 - 2018 (4) & -17.29 & 0.42 & 0.01 & 22.12\\
Mexico & 1997 - 2021 (19) & -3.08 & -0.11 & -0.15 & 2.12\\
Moldova & 1998 - 2019 (19) & 30.14 & 0.00 & -0.18 & -10.05\\
Mongolia & 2008 - 2020 (10) & 9.41 & -0.18 & -0.09 & -0.30\\
\addlinespace
Morocco & 2000 - 2021 (17) & -316.72 & -1.12 & -0.27 & -2.72\\
Netherlands & 1997 - 2021 (17) & 5.53 & -0.21 & -0.09 & -1.44\\
New Zealand & 1997 - 2019 (17) & 12.22 & 0.03 & -0.01 & -0.73\\
Nicaragua & 2008 - 2018 (11) & -2.80 & 0.12 & -0.14 & 5.15\\
Niger & 1997 - 2019 (19) & -0.64 & -0.26 & -0.87 & -4.68\\
\addlinespace
Norway & 1982 - 2021 (32) & -7.35 & -0.25 & -0.07 & 1.58\\
Peru & 2009 - 2021 (11) & -20.34 & 1.05 & -0.30 & -4.78\\
Philippines & 1997 - 2022 (20) & -13.42 & 0.35 & -0.20 & -6.72\\
Poland & 1997 - 2021 (14) & 654.60 & 1.38 & -0.06 & -16.69\\
Portugal & 1997 - 2022 (15) & 95.33 & -0.11 & -0.08 & 37.63\\
\addlinespace
Qatar & 2004 - 2017 (10) & -0.20 & -0.29 & -0.21 & 0.83\\
Romania & 1997 - 2020 (13) & -12.57 & 0.16 & -0.15 & -3.68\\
Russia & 1997 - 2017 (12) & 3.33 & -0.51 & -0.16 & -2.27\\
Saudi Arabia & 2005 - 2009 (3) & 183.74 & -120.27 & 0.98 & 0.82\\
Senegal & 2018 - 2021 (3) & -15.59 & -2.01 & -1.31 & -0.37\\
\addlinespace
Serbia & 1999 - 2021 (21) & 8.99 & 1.17 & -0.66 & 1.57\\
Slovakia & 1997 - 2021 (17) & 180.60 & -0.15 & -0.17 & -2.61\\
Slovenia & 1999 - 2021 (15) & -6.24 & -0.11 & -0.07 & -5.12\\
South Africa & 1997 - 2022 (18) & 97.77 & -0.93 & -0.13 & 1.38\\
South Korea & 1997 - 2020 (14) & 8.25 & -0.19 & -0.03 & -2.50\\
\addlinespace
Spain & 1996 - 2021 (21) & -11.36 & -0.02 & -0.11 & 0.38\\
Sweden & 1980 - 2021 (32) & -1.67 & -0.10 & -0.13 & -2.41\\
Switzerland & 1993 - 2020 (20) & 56.23 & -1.70 & -0.08 & 0.30\\
Tunisia & 1997 - 2011 (12) & 20.84 & 4.70 & -0.17 & -4.94\\
Turkey & 2011 - 2015 (5) & -8.65 & -2.52 & -0.54 & 0.00\\
\addlinespace
USA & 1981 - 2021 (33) & 10.38 & -0.18 & -0.10 & 2.65\\
Ukraine & 1998 - 2019 (19) & 0.21 & -0.32 & -0.10 & 1.51\\
United Kingdom & 1981 - 2021 (30) & 2.03 & -0.03 & -0.20 & 0.17\\
Uruguay & 2017 - 2017 (1) & 6.73 & 0.56 & 0.02 & 0.03\\
Uzbekistan & 2012 - 2021 (8) & 9.93 & -0.28 & -0.14 & 2.85\\
\addlinespace
Vanuatu & 2003 - 2007 (3) & 94333.86 & -0.69 & -0.19 & 7.71\\
Venezuela & 2000 - 2019 (18) & -43.75 & 0.75 & -0.15 & 5.62\\
\bottomrule
\end{tabular}
